DeepTest: Automated Testing of Deep-Neural-Network-driven Autonomous Cars

Recent advances in Deep Neural Networks (DNNs) have led to the development of DNN-driven autonomous cars that, using sensors like camera, LiDAR, etc., can drive without any human intervention. Most major manufacturers including Tesla, GM, Ford, BMW, and Waymo/Google are working on building and testing different types of autonomous vehicles. The lawmakers of several US states including California, Texas, and New York have passed new legislation to fast-track the process of testing and deployment of autonomous vehicles on their roads. However, despite their spectacular progress, DNNs, just like traditional software, often demonstrate incorrect or unexpected corner case behaviors that can lead to potentially fatal collisions. Several such real-world accidents involving autonomous cars have already happened including one which resulted in a fatality. Most existing testing techniques for DNN-driven vehicles are heavily dependent on the manual collection of test data under different driving conditions which become prohibitively expensive as the number of test conditions increases. In this paper, we design, implement and evaluate DeepTest, a systematic testing tool for automatically detecting erroneous behaviors of DNN-driven vehicles that can potentially lead to fatal crashes. First, our tool is designed to automatically generated test cases leveraging real-world changes in driving conditions like rain, fog, lighting conditions, etc. DeepTest systematically explores different parts of the DNN logic by generating test inputs that maximize the numbers of activated neurons. DeepTest found thousands of erroneous behaviors under different realistic driving conditions (e.g., blurring, rain, fog, etc.) many of which lead to potentially fatal crashes in three top performing DNNs in the Udacity self-driving car challenge.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = main

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		$(name).out \
		psfig.aux \
		*.bbl \
		*.pdfsync

#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> guidedimages.tex <==
\begin{table}[htbp]
  \centering
  \scriptsize
  \caption{\small Violations from guided search}
  
    \begin{tabular}{c|c|c}
    \toprule
 \textbf{baseline} &\textbf{generated image}& \textbf{transformations} \\ \midrule

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425443687382945_arrow}.jpg} &

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425443687382945.jpg_178_arrow}.jpg} & \makecell{Averaging blur:4x4;\\Translation:128,128;}  \\ \midrule
 

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425478693111335_arrow}.jpg} &

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425478693111335.jpg_205_arrow}.jpg} & \makecell{Scale:0.6;\\ Contrast:0.4;}  \\ \midrule

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425478693111335_arrow}.jpg}&

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425478693111335.jpg_217_arrow}.jpg} & \makecell{Scale:0.6;\\ Brightness:75;}  \\ \midrule






\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425443687382945_arrow}.jpg}&

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425443687382945.jpg_185_arrow}.jpg} & \makecell{Brightness:99;\\ Scale:1.7; \\ Scale:1.7; \\ Brightness:46;}  \\ \midrule

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425451188093502_arrow}.jpg}&

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425451188093502.jpg_190_arrow}.jpg} & \makecell{Scale:1.3; \\ Translation:74,74;}  \\ \midrule

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425451188093502_arrow}.jpg}&

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425451188093502.jpg_191_arrow}.jpg} & \makecell{ Scale:1.3; \\ Translation:74,74; \\ Gaussian blur:3x3; \\Brightness:85;}  \\ \midrule

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425508699129652_arrow}.jpg}&

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425508699129652.jpg_213_arrow}.jpg} & \makecell{Brightness:100; \\ Gaussian blur:5x5; \\ Scale:1.3; \\ Brightness:-27; \\ Median blur:3; \\ Brightness:-86;}  \\ \midrule

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425638721344700_arrow}.jpg}&

\includegraphics[width=0.1\textwidth, height=0.1\textwidth, valign=c]{{./figures/guided/guided_1479425638721344700.jpg_225_arrow}.jpg} & \makecell{Scale:0.5; \\ Averaging blur:5x5;}  \\ 

 \bottomrule
    \end{tabular}%
  \label{tab:guided}%
\end{table}%


==> listofitems.tex <==
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.3}                              %
%                                                                    %
\def\loidate                  {2016/11/18}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% --------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
% %     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% --------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% email: unbonpetit@openmailbox.org
%        Commentaires, suggestions et signalement de bugs bienvenus !
%        Comments, bug reports and suggestions are welcome.
% --------------------------------------------------------------------
% L'extension listofitems est compos\'ee des 7 fichiers suivants :
%   - code               : listofitems            (.tex et .sty)
%   - manuel en francais : listofitems-fr         (.tex et .pdf)
%   - manuel en anglais  : listofitems-en         (.tex et .pdf)
%   - fichier lisezmoi   : README
% --------------------------------------------------------------------
\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% gestion des erreurs %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% v\'erification de la pr`'esence de etex %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\edef\__tempa{\meaning\eTeXversion}\edef\__tempb{\string\eTeXversion}%
\ifx\__tempa\__tempb
	\endgroup
\else
	\endgroup
	\loi_error{You are not using an eTeX engine, listofitems cannot work.}%
	\expandafter\loi_restorecatcode\expandafter\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---- macros de d\'eveloppement et de manipulation d'arguments
\chardef\loi_stop=0
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_swaparg#1#2{#2{#1}}
\long\def\loi_exparg#1#2{\expandafter\loi_swaparg\expandafter{#2}{#1}}
\long\def\loi_expafternil#1\_nil{\begingroup\def\loi_temp{\endgroup#1}\expandafter\loi_temp}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\begingroup\def\loi_temp{\endgroup#1}\loi_argcsname_i}
\def\loi_argcsname_i#1{\expandafter\loi_temp\csname#1\endcsname}

%--- macros de test
\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_i{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_i}
\long\def\loi_ifcs#1{% #1 est-il une sc ?
	\loi_ifempty{#1}
		\loi_second% si #1 est vide, faux
		{\loi_ifspacefirst{#1}
			\loi_second% si espace en 1er, faux
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\begingroup \escapechar`\_
					\if\expandafter\loi_firsttonil\string#1\_nil\expandafter\loi_firsttonil\string\relax\_nil
						\endgroup\expandafter\loi_first
					\else
						\endgroup\expandafter\loi_second
					\fi
				}
				\loi_second% si plusieurs tokens, faux
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }\loi_second\loi_first}

%--- macro de type for
%      Voir codes 150 \`a 155 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 175 \`a 184 du livre "Apprendre \`a programmer en TeX"
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}\edef\loi_sgncmp{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
	\loi_argcsname\loi_fornum_i{loi_fornum_\string#1\expandafter}\expandafter{\number\numexpr#3\expandafter}\loi_sgncmp#1%
}
\long\def\loi_fornum_i#1#2#3#4#5#6{\def#1{\unless\ifnum#5#3#2\relax\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}\fi}#1}

%--- macros retirant les espaces extr\^emes
%      Voir codes 320 \`a 324 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 339 \`a 343 de "Apprendre \`a programmer en TeX"
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_i\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_i#1 #2\_nil{\loi_ifempty{#1}}
\expandafter\def\expandafter\loi_gobspace\space{}
\def\loi_removefirstspaces{\romannumeral\loi_removefirstspaces_i}
\long\def\loi_removefirstspaces_i#1{\loi_ifspacefirst{#1}{\expandafter\loi_removefirstspaces_i\expandafter{\loi_gobspace#1}}{\loi_stop#1}}
\edef\loi_restorezerocatcode{\catcode0=\number\catcode0 \relax}
\catcode0 12
\long\def\loi_removelastspaces#1{\romannumeral\loi_removelastspaces_i#1^^00 ^^00\_nil}
\long\def\loi_removelastspaces_i#1 ^^00{\loi_removelastspaces_ii#1^^00}
\long\def\loi_removelastspaces_ii#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_i#1^^00 ^^00\_nil}{\loi_stop#1}}
\loi_restorezerocatcode
\long\def\loi_removeextremespaces#1{% #1=texte o\`u les espaces extr\^emes sont retir\'es
	\romannumeral\expandafter\expandafter\expandafter\loi_removelastspaces\expandafter\expandafter\expandafter
	{\expandafter\expandafter\expandafter\loi_stop\loi_removefirstspaces{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_i}
\def\setsepchar_i{\loi_ifx{[\loi_nxttok}\setsepchar_ii{\setsepchar_ii[/]}}
\long\def\setsepchar_ii[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_ii[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % r\'einitaliser niveau initial \`a 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_iv1{,}%
			}
			{\readlist_iv1{#2}}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de s\'eparation
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2#3{% #1=macroname  #2=liste d'index  #3=profondeur max --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{\loi_stop{}{}}
		{\loi_normalizeindex_i1{}{#3}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_i#1#2#3#4#5,{% #1=compteur de profondeur #2=index pr\'ec\'edents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_iii#2\loi_quark}% supprimer la derni\`ere virgule
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}}% si profondeur trop grande
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_ii{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_ii#1#2#3{\loi_exparg\loi_normalizeindex_i{\number\numexpr#2+1}{#3#1,}}% #1=index \`a rajouter  #2=compteur de profondeur #3=index pr\'ec\'edents
\def\loi_normalizeindex_iii#1,\loi_quark{\loi_stop{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_i{#1},}\loi_invalidindex_i{#1}{#2}}
\def\loi_invalidindex_i#1#2{\loi_invalidindex_ii#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_ii#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{\loi_stop{#1[#3]#2}{#3}}% #4= index ignor\'es

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{%
	\let\loi_def\gdef \let\loi_edef\xdef \def\loi_let{\global\let}%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\loi_let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\def\readlist{%
	\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\long\def\readlist_i#1#2{% #1=macro stockant les \'el\'ements  #2=liste des \'el\'ements
	\loi_ifcs{#2}
		{\loi_exparg{\readlist_i#1}{#2}}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_argcsname\loi_let{\loi_listname nest}\nestdepth
		\loi_argcsname\loi_def{\loi_listname[]}{#2}% la liste enti\`ere
		\loi_argcsname\loi_def{\loi_listname sep[]}{}% s\'eparateur vide
		\loi_ifempty{#2}
			{\loi_def#1[##1]{}%
			\loi_argcsname\loi_def{\loi_listname len}{0}\loi_argcsname\loi_def{\loi_listname len[0]}{0}%
			\loi_error{Empty list ignored, nothing to do}%
			}
			{\loi_edef#1[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname}}%
			\loi_argcsname\loi_edef{\loi_listname sep}[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname sep}}%
			\readlist_ii{#2}%
			\loi_argcsname\loi_argcsname\loi_let{\loi_listname len}{\loi_listname len[0]}% longueur du niveau 0
			}%
		}%
}
\def\loi_auxmacrolistitem#1#2#3{%
	\expandafter\expandafter\expandafter\loi_stop\csname#3[#2]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}
\def\readlist_ii{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_iii\loi_currentsep||\_nil
}
\long\def\readlist_iii#1||#2\_nil#3{\readlist_iv1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un \'el\'ement vide pour le test ifempty ci dessous
\long\def\readlist_iv#1#2{% #1=compteur d'index  #2=liste d'\'el\'ements \`a examiner
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafternil\readlist_vi{#2}{}\_nil\loi_currentsep||\loi_quark||#2\_nil{#1}}% aller isoler le 1er item
}
\long\def\readlist_v#1#2{\readlist_vi{#2}{}#1||\loi_quark||#2\_nil}% #1=liste s\'eparateurs (s\'ep=||)  #2=chaine de tokens
\long\def\readlist_vi#1#2#3||{% #1=liste restante   #2=dernier <sep utile>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}
		{\loi_ifempty{#2}% si #1 vide, aucun <sep utile> n'a \'et\'e trouv\'e, il reste \`a lire "<liste compl\`ete>\_nil"
			{\long\def\readlist_vii##1\_nil##2{\loi_exparg{\readlist_ix{##2}{}}{\loi_gobarg##1}{#2}}}% ##2=compteur d'index
			{\long\def\readlist_vii##1#2{\loi_exparg\readlist_viii{\loi_gobarg##1}\relax}%
			\long\def\readlist_viii##1##2\_nil##3{\loi_exparg{\readlist_ix{##3}}{\loi_gobarg##2}{##1}{#2}}% ##3=compteur d'index
			}%
		\readlist_vii\relax% le \relax meuble l'argument d\'elimit\'e
		}
		{\long\def\readlist_vii##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_vi{#1}{#2}}% recommencer avec le m\^eme <sep utile>
				{\readlist_vi{##1#3}{#3}}% sinon raccourcir <liste restante> et <sep courant>:=<sep utile>
			}%
		\readlist_vii#1#3\_nil
		}%
}
\long\def\readlist_ix#1#2#3{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extr\^emes
		{\loi_exparg{\loi_exparg{\readlist_x{#1}{#2}}}{\loi_removeextremespaces{#3}}}% red\'efinir l'\'el\'ement courant
		{\readlist_x{#1}{#2}{#3}}%
}
\long\def\readlist_x#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant   #4=sep utilis\'e
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_iv{#1}{#2}}% si l'on n'ignore pas les \'el\'ements vides :
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation de l'item ctuel \`a la macro
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel \`a la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_ii{#3}% recommencer avec l'\'el\'ement courant
			}
			{}%
		\loi_exparg\readlist_iv{\number\numexpr#1+1}{#2}% puis chercher l'\'el\'ement suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\romannumeral\loi_ifempty{#2}
		{\expandafter\expandafter\expandafter\loi_stop\csname\loi_macroname#1len[0]\endcsname}
		{\loi_exparg\listlen_i{\romannumeral-`\.\loi_macroname#1}{#2}}%
}
\def\listlen_i#1#2{% #1=macro name   #2=index non normalis\'e    prendre <profondeur max-1>
	\loi_exparg{\expandafter\listlen_ii\romannumeral\loi_normalizeindex{#1}{#2}}{\number\numexpr\csname#1nest\endcsname-1}{#1}%
}
\def\listlen_ii#1#2#3{% #1=err   #2=index normalis\'e  #3=macroname
	\expandafter\expandafter\expandafter\loi_stop\csname#3len[#2,0]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_i{\noexpand\foreachitem_iii\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_ii
}
\def\foreachitem_ii{\loi_ifx{\loi_nxttok[}\foreachitem_i{\foreachitem_i[]}}
\def\foreachitem_iii#1#2#3[#4]{% prendre <profondeur max-1>
	\loi_exparg{\expandafter\foreachitem_iv\romannumeral\loi_normalizeindex{#3}{#4}}{\number\numexpr\csname#3nest\endcsname-1}#1{#2}{#3}%
}
\def\foreachitem_iv#1#2{\loi_ifempty{#2}{\foreachitem_v{#1}{}}{\foreachitem_v{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_v#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associ\'e  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_i}{\let\showitems_cmd\loi_identity\showitems_i}}
\def\showitems_i#1{\def\showitems_ii{\showitems_iv#1}\futurelet\loi_nxttok\showitems_iii}
\def\showitems_iii{\loi_ifx{\loi_nxttok[}\showitems_ii{\showitems_ii[]}}
\def\showitems_iv#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % r\'eglages identiques \`a LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir codes 251 \`a 254 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
		\hbox{% et pages 271 \`a 274 de "Apprendre \`a programmer en TeX"
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par d\'efaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}{\global\let}%
}
\def\itemtomacro_i#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% r\'eglages par d\'efaut %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\setsepchar{,}
\reademptyitems

\loi_restorecatcode
\endinput

######################################################################
#                             Historique                             #
######################################################################

v1.0  19/8/2016
      - Premi\`ere version publique

v1.1  01/09/2016
      - Stockage des s\'eparateurs dans <macrolist>sep
      - bug corrig\'e dans \loi_restorecatcode

v1.2  22/10/2016
      - macros \greadlist et \gitemtomacro pour la globalit\'e

v1.3  18/11/2016
      - bugs corrig\'es dans la gestion de la globalit\'e

==> ncoverage.tex <==
\subsection{Neuron coverage}
Neuron coverage measures the percentage of number of unique neurons that get activated of the total number of neurons in the DNN given test input(s).
Each neuron's output affects the final output of a DNN. If a neuron outputs a value higher than a threshold, it is considered activated, i.e., it is detecting some feature. 
As different types of neuron output different type of values (\ie single value, multiple values organized in a multidimensional array), we discuss the detail how we handle the output of different types of neurons in the following.
(1) In the case of a neuron in fully-connected layers, the output is a single scalar, which we can directly compare it with the threshold to determine the activation.
(2) In the case of convolutional layers, each neuron's output is no longer a single scalar value. 
Specifically, the output of a neuron is the result of applying a convolutional kernel across the input space, which produces a multidimensional feature map~\cite{hijazi2015using}.
The first layer in Figure~\ref{subfig:cnn} illustrates applying one convolutional kernel (with size 3$\times$3) to the image space (with size 6$\times$6) that produces the feature map of size 3$\times$3 in the succeeding layer.
In real world self-driving CNN such as that proposed by Nvidia~\cite{bojarski2016end}, convolution layers consist many convolutional kernels (\cite{bojarski2016end} paper has 64 kernels in its 5-th layer, resulting in 64 feature maps denoting the outputs of 64 neurons respectively).
We take the average of the feature map to convert the multidimensional output of a neuron into a scalar, which enables comparison to the threshold.
(3) In the case of RNN/LSTM, the intermediate neurons are unrolled that output a sequence of outputs (Figure~\ref{subfig:rnn} right) or not-unrolled that output a single value (Figure~\ref{subfig:rnn} left).
In the unrolled layers, we treat each neuron in the unrolled layers as a separate individual neuron and compute their neuron coverage. 
In the not-unrolled layers, the neurons are incrementally fed with a sequence of inputs and output a single value after the last input has been fed. 
In this case, we only consider the output of this single neuron and compute its output to determine the coverage after finishing processing a sequence of inputs.


==> tab1.tex <==
% Table generated by Excel2LaTeX from sheet 'result (2)'
\begin{table*}[htbp]
  \centering
  \scriptsize
  \caption{Add caption}
    \begin{tabular}{cllrrrl}
          &       &       & \multicolumn{2}{c}{t-test } & \multicolumn{2}{c}{cohen's D} \\
    \multicolumn{1}{l}{model} & sub-model & tranformation   & \multicolumn{1}{l}{  mean difference  } & \multicolumn{1}{l}{  mean difference (\%)  } & \multicolumn{1}{l}{  d\$estimate  } &   d\$magnitude \\
    \multirow{7}[0]{*}{Epoch} &       & rotation   & 61.12 & 2.44\% & 1.45  &   Large \\
          &       & translation   & 71.47 & 2.86\% & 1.83  &   Large \\
          &       & shear   & 111.09 & 4.44\% & 2.33  &   Large \\
          &       & contrast   & 66.45 & 2.66\% & 1.59  &   Large \\
          &       & brightness   & 90.52 & 3.62\% & 1.89  &   Large \\
          &       & blur   & 16.42 & 0.66\% & 0.42  &   Small \\
          &       & scale   & 22.85 & 0.91\% & 0.67  &   Medium \\
    \multirow{21}[0]{*}{Rambo} & s1    &   rotation   & 71.283 & 4.39\% & 4.52  &   large \\
          & s1    &   translation   & 143.707 & 8.84\% & 11.47 &   large \\
          & s1    &   shear   & 87.623 & 5.39\% & 5.82  &   large \\
          & s1    &   contrast   & 48.283 & 2.97\% & 4.43  &   large \\
          & s1    &   brightness   & 66.81 & 4.11\% & 4.67  &   large \\
          & s1    &   blur   & 19.349 & 1.19\% & 1.27  &   large \\
          & s1    &   scale   & 3.177 & 0.20\% & 0.24  &   small \\
          & s2    &   rotation   & 16.772 & 0.44\% & 0.83  &   large \\
          & s2    &   translation   & 172.18 & 4.53\% & 7.46  &   large \\
          & s2    &   shear   & 120.134 & 3.16\% & 4.88  &   large \\
          & s2    &   contrast   & 98.703 & 2.60\% & 3.02  &   large \\
          & s2    &   brightness   & 106.773 & 2.81\% & 2.76  &   large \\
          & s2    &   blur   & 23.976 & 0.63\% & 0.89  &   large \\
          & s2    &   scale   & 5.108 & 0.13\% & 0.23  &   small \\
          & s3    &   rotation   & 872.75 & 6.48\% & 0.44  &   small \\
          & s3    &   translation   & 1879.198 & 13.95\% & 1.24  &   large \\
          & s3    &   shear   & 11659.356 & 86.54\% & 7.88  &   large \\
          & s3    &   contrast   & 81.787 & 0.61\% & 0.04  &   negligible \\
          & s3    &   brightness   & 620.451 & 4.61\% & 0.29  &   small \\
          & s3    &   blur   & 562.189 & 4.17\% & 0.23  &   small \\
          & s3    &   scale   & 105.993 & 0.79\% & 0.05  &   negligible \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> tables/dnn.tex <==
%!TEX root = ../main.tex

\begin{table}[htbp]
  \centering
  \scriptsize
  \caption{\small Details of DNNs and datasets used to evaluate DeepTest, as taken from Udacity Self Driving Car Challenge 2~\cite{dataset}\wu}
\begin{threeparttable}
    \centering
    %\begin{tabular}{l|l|l|l|l|l}
    \begin{tabular}{lllll}
        &  & \textbf{No. of} & \textbf{Reported} & \textbf{Our} \\
\textbf{Model} & \textbf{Sub-Model} & \textbf{Neurons}& \textbf{MSE} & \textbf{MSE} \\
\toprule
\multirow{2}[0]{*}{\textbf{\chauf}} & CNN & 1427 & \multirow{2}[0]{*}{0.06} & \multirow{2}[0]{*}{0.06}\\
          & LSTM & 513 & &  \\
          
\midrule

\multirow{3}[0]{*}{\textbf{\rambo}} & S1(CNN)  & 1625 & \multirow{3}[0]{*}{0.06} & \multirow{3}[0]{*}{0.05}\\
          
          & {S2}(CNN)   & 3801 & & \\
          & {S3}(CNN)   & 13473 & & \\
          
\midrule
    \textbf{\epoch} &  CNN    & 2500 & 0.08 & 0.10 \\
    \bottomrule
    
    \end{tabular}%
    \begin{tablenotes}
      \footnotesize
      \item[\wu]  dataset HMB\_3.bag~\cite{dataset}
    \end{tablenotes}
\end{threeparttable}
  \label{tab:dnn}%
\end{table}%


==> tables/rq2.tex <==
% Table generated by Excel2LaTeX from sheet 'result (2)'
\begin{table*}[htbp]
  \centering
  \setlength{\tabcolsep}{4pt}
    \scriptsize
    \renewcommand{\arraystretch}{.9}
  \caption{Add caption}
    \begin{tabular}{cllrrrl}
          &       &       & \multicolumn{2}{c}{t-test } & \multicolumn{2}{c}{cohen's D} \\
    \multicolumn{1}{l}{model} & sub-model & tranformation   & \multicolumn{1}{l}{  mean difference  } & \multicolumn{1}{l}{  mean difference (\%)  } & \multicolumn{1}{l}{  d\$estimate  } &   d\$magnitude \\
    \multirow{7}[0]{*}{Epoch} &       & rotation   & 61.12 & 2.44\% & 1.45  &   Large \\
          &       & translation   & 71.47 & 2.86\% & 1.83  &   Large \\
          &       & shear   & 111.09 & 4.44\% & 2.33  &   Large \\
          &       & contrast   & 66.45 & 2.66\% & 1.59  &   Large \\
          &       & brightness   & 90.52 & 3.62\% & 1.89  &   Large \\
          &       & blur   & 16.42 & 0.66\% & 0.42  &   Small \\
          &       & scale   & 22.85 & 0.91\% & 0.67  &   Medium \\
    \multirow{21}[0]{*}{Rambo} & s1    &   rotation   & 71.283 & 4.39\% & 4.52  &   large \\
          & s1    &   translation   & 143.707 & 8.84\% & 11.47 &   large \\
          & s1    &   shear   & 87.623 & 5.39\% & 5.82  &   large \\
          & s1    &   contrast   & 48.283 & 2.97\% & 4.43  &   large \\
          & s1    &   brightness   & 66.81 & 4.11\% & 4.67  &   large \\
          & s1    &   blur   & 19.349 & 1.19\% & 1.27  &   large \\
          & s1    &   scale   & 3.177 & 0.20\% & 0.24  &   small \\
          & s2    &   rotation   & 16.772 & 0.44\% & 0.83  &   large \\
          & s2    &   translation   & 172.18 & 4.53\% & 7.46  &   large \\
          & s2    &   shear   & 120.134 & 3.16\% & 4.88  &   large \\
          & s2    &   contrast   & 98.703 & 2.60\% & 3.02  &   large \\
          & s2    &   brightness   & 106.773 & 2.81\% & 2.76  &   large \\
          & s2    &   blur   & 23.976 & 0.63\% & 0.89  &   large \\
          & s2    &   scale   & 5.108 & 0.13\% & 0.23  &   small \\
          & s3    &   rotation   & 872.75 & 6.48\% & 0.44  &   small \\
          & s3    &   translation   & 1879.198 & 13.95\% & 1.24  &   large \\
          & s3    &   shear   & 11659.356 & 86.54\% & 7.88  &   large \\
          & s3    &   contrast   & 81.787 & 0.61\% & 0.04  &   negligible \\
          & s3    &   brightness   & 620.451 & 4.61\% & 0.29  &   small \\
          & s3    &   blur   & 562.189 & 4.17\% & 0.23  &   small \\
          & s3    &   scale   & 105.993 & 0.79\% & 0.05  &   negligible \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> tables/rq2_baseline.tex <==
%!TEX root = ../main.tex
% Table generated by Excel2LaTeX from sheet 'RQ2 (2)'
% \begin{table}[htbp]
%   \centering

%     \caption{Add caption}
{\scriptsize
\begin{tabular}{lrrr}

\multicolumn{4}{c}{\textbf{\small Increase in Neurons Coverage}} \\
\multicolumn{4}{c}{\textbf{\small from the originial  images by each transformation}} \\
\toprule
\textbf{Tranformation} & \textbf{Epoch} & \textbf{Rambo} & \textbf{Chauffeur} \\
	                   &   &  \textbf{(S1,S2,S3)} &  \textbf{(CNN, LSTM)} \\
\toprule
Rotation   & 82.59 & (71.28, 16.77, \underline{872.75}) & (192.19, \underline{10.54}) \\
  		   & 169\% & (14\%, 4\%, \underline{66\%}) 		&  (124\%, \underline{2\%})\\
\midrule
Translation   & 74.81 & (143.71, 172.18, 1879.20) 	& (141.97, \underline{9.31}) \\
			  & 153\% & (30\%, 39\%, 143\%) 	& (91\%, \underline{2\%}) \\
\midrule
Shear   & 157.87 & (49.78, 128.09, 4252.03) 		& (174.98, \underline{10.14}) \\
	    & 323\% & (10\%, 29\%, 323\%) 		& (113\%, \underline{2\%}) \\
\midrule

Contrast   & 71.32 & (48.28, 98.70, \wu{81.79}) 	& (119.09, \underline{9.36}) \\
		   & 146\% & (10\%, 22\%, \wu{6\%}) 	& (77\%, \underline{2\%}) \\
\midrule
Brightness   & 109.49 & (66.81, 106.77, \underline{620.45}) 	& (115.67, \wu{4.96}) \\
             & 224\% & (14\%, 24\%, \underline{47\%}) 	& (74\%, \wu{1\%}) \\
\midrule
Blur   & \underline{8.09}  & (19.35, 23.98, \underline{562.19}) & (45.78, \wu{0.94}) \\
       & \underline{17\%}  & (4\%, 5\%, \underline{43\%}) & (29\%, \wu{0.18\%}) \\
\midrule
Scale   & 43.34 & (\underline{3.18}, \underline{5.11}, \wu{105.99}) & (\wu{1.22}, \wu{2.75}) \\
        & 89\% & (\underline{1\%}, \underline{1\%}, \wu{8\%}) & (\wu{0.78\%}, \wu{0.54\%}) \\
\bottomrule
\end{tabular}%

{All the numbers are statistically significant; Numbers with \wu{} stands for neglighble Cohen's D effect, while \underline{undeline} is for small effect. 
All the other numbers show large effect.}
}
%        \label{tab:addlabel}%
% \end{table}

==> tables/rq4_per_threshold.tex <==
%!TEX root = ../main.tex

% Table generated by Excel2LaTeX from sheet 'err_varying_threshold'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{\small{Number of unique erroneous behavior reported at different thresholds}}
    \label{tab:rq4Th}%
    \begin{tabular}{r|rrrrr|rr}
  \toprule
      Threshold    & \multicolumn{5}{c|}{Parametric Transformation} & \multicolumn{2}{c}{Non-parametric} \\
        \wrt  & \multicolumn{5}{c|}{Threshold on MSE differences \wrt baseline} &  \multicolumn{2}{c}{Transformation}  \\
  MSE & 0.01  & 0.02  & 0.03  & 0.04  & 0.05  & \multicolumn{1}{l}{Rain} & \multicolumn{1}{l}{Fog} \\
  \midrule
    1     & 3538  & 4038  & 5106  & 5479  & 6619  & 1462  & 2891 \\
    2     & 895   & 1021  & 1296  & 1395  & 1740  & 371   & 357 \\
    3     & 284   & 343   & \Red{470} & 517   & 697   & \Red{82} & \Red{110} \\
    4     & 100   & 151   & 230   & 245   & 306   & 21    & 59 \\
    5     & 32    & 40    & 67    & 78    & 113   & 3     & 15 \\
  \bottomrule
    \end{tabular}%
\end{table}%

